Benchmarking Safety Monitors for Image Classifiers with Machine Learning

High-accurate machine learning (ML) image classifiers cannot guarantee that they will not fail at operation. Thus, their deployment in safety-critical applications such as autonomous vehicles is still an open issue. The use of fault tolerance mechanisms such as safety monitors is a promising direction to keep the system in a safe state despite errors of the ML classifier. As the prediction from the ML is the core information directly impacting safety, many works are focusing on monitoring the ML model itself. Checking the efficiency of such monitors in the context of safety-critical applications is thus a significant challenge. Therefore, this paper aims at establishing a baseline framework for benchmarking monitors for ML image classifiers. Furthermore, we propose a framework covering the entire pipeline, from data generation to evaluation. Our approach measures monitor performance with a broader set of metrics than usually proposed in the literature. Moreover, we benchmark three different monitor approaches in 79 benchmark datasets containing five categories of out-of-distribution data for image classifiers: class novelty, noise, anomalies, distributional shifts, and adversarial attacks. Our results indicate that these monitors are no more accurate than a random monitor. We also release the code of all experiments for reproducibility.

==> sections/tables/anomaly_tables.tex <==
\begin{table}[htb!]
\centering
\caption{Comparing data-based monitors for CIFAR-10 and GTSRB datasets with \textbf{anomaly}.}
\resizebox{\columnwidth}{!}{%
\label{table_anomaly}
\begin{tabular}{llllllll}
\toprule
\multicolumn{8}{c} {CIFAR-10}\\
\toprule
Variation &                                             Method &                                                MCC &                                                FPR &                                                FNR &                                          Pr &                                             Re &                                           F1 \\
\midrule
     pixel trap (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
    \begin{tabular}{@{}c@{}}\textbf{0.6} \\ 0.02 \\ -0.17\end{tabular} &  %1,2,3
    \begin{tabular}{@{}c@{}}\textbf{0.0} \\ 1.0 \\ 0.43\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ \textbf{0.0} \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.97} \\ 0.14 \\ 0.07\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ \textbf{1.0} \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.9} \\ 0.04 \\ 0.59\end{tabular} \\

\midrule

 row add logic  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 \begin{tabular}{@{}c@{}}-0.01 \\ \textbf{0.01} \\ \textbf{0.01}\end{tabular} &  %3,1,1
 \begin{tabular}{@{}c@{}}0.42 \\ 1.0 \\ \textbf{0.18}\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ \textbf{0.0} \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.14 \\ 0.14 \\ \textbf{0.15}\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ \textbf{1.0} \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.62 \\ 0.04 \\ \textbf{0.74}\end{tabular} \\
 
 \midrule
 
 shifted pixel  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 \begin{tabular}{@{}c@{}}\textbf{0.16} \\ 0.0 \\ 0.0\end{tabular} &  %1,2,2
 \begin{tabular}{@{}c@{}}0.21 \\ 1.0 \\ \textbf{0.19}\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ \textbf{0.0} \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.24} \\ 0.14 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ \textbf{1.0} \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.76} \\ 0.04 \\ 0.74\end{tabular} \\
 
\bottomrule
\bottomrule
\multicolumn{8}{c} {GTSRB}\\
\toprule
Variation &                                             Method &                                                MCC &                                                FPR &                                                FNR &                                          Pr &                                             Re &                                           F1 \\
\midrule
    pixel trap  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
    \begin{tabular}{@{}c@{}}\textbf{0.6} \\ -0.01 \\ -0.01\end{tabular} &  %1,2,2
    \begin{tabular}{@{}c@{}}\textbf{0.09} \\ 0.85 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ \textbf{0.02}\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.66} \\ 0.19 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ \textbf{0.98}\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.87} \\ 0.27 \\ 0.09\end{tabular} \\
    
\midrule

 row add logic  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 \begin{tabular}{@{}c@{}}-0.02 \\ \textbf{0.03} \\ 0.02\end{tabular} &  %3,1,2
 \begin{tabular}{@{}c@{}}0.73 \\ 0.81 \\ \textbf{0.97}\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.29} \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.19 \\ \textbf{0.2} \\ \textbf{0.2}\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ \textbf{0.98}\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.38} \\ 0.32 \\ 0.11\end{tabular} \\
 
 \midrule
 
 shifted pixel  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 \begin{tabular}{@{}c@{}}\textbf{0.02} \\ 0.01 \\ \textbf{0.02}\end{tabular} &  %1,2,1
 \begin{tabular}{@{}c@{}}\textbf{0.69} \\ 0.83 \\ 0.97\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ \textbf{0.02}\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.2} \\ \textbf{0.2} \\ \textbf{0.2}\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ \textbf{0.98}\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.42} \\ 0.29 \\ 0.11\end{tabular} \\
\bottomrule
\end{tabular}
}
\end{table}







%\begin{table}[htb!]
%\centering

%\caption{Comparing data-based monitors for cifar10 dataset with different types of anomalies.}
%\resizebox{\columnwidth}{!}{%

%\label{table_anomaly_cifar10}
%\begin{tabular}{llllllll}
%\toprule
%                Variation &                                             Method &                                                MCC &                                                FPR &                                                FNR &                                          Pr &                                             Re &                                           F1 \\
%\midrule
%    pixel trap (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%    \begin{tabular}{@{}c@{}}0.6 \\ 0.02 \\ -0.17\end{tabular} &  %1,2,3
%    \begin{tabular}{@{}c@{}}0.0 \\ 1.0 \\ 0.43\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.97 \\ 0.14 \\ 0.07\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.9 \\ 0.04 \\ 0.59\end{tabular} \\

%\midrule

% row add logic  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.01 \\ 0.01 \\ 0.01\end{tabular} &  %3,1,1
% \begin{tabular}{@{}c@{}}0.42 \\ 1.0 \\ 0.18\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.14 \\ 0.14 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.62 \\ 0.04 \\ 0.74\end{tabular} \\
 
% \midrule
 
% shifted pixel  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.16 \\ 0.0 \\ 0.0\end{tabular} &  %1,2,2
% \begin{tabular}{@{}c@{}}0.21 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.24 \\ 0.14 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.76 \\ 0.04 \\ 0.74\end{tabular} \\
 
% \midrule
 
%    pixel trap  (1) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%    \begin{tabular}{@{}c@{}}0.51 \\ 0.02 \\ -0.52\end{tabular} &  %1,2,3
%    \begin{tabular}{@{}c@{}}0.02 \\ 1.0 \\ 0.84\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.77 \\ 0.14 \\ 0.04\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.88 \\ 0.04 \\ 0.22\end{tabular} \\
    
%\midrule

% row add logic  (1) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.0 \\ 0.0 \\ 0.11\end{tabular} &  %2,2,1
% \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.09\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.14 \\ 0.14 \\ 0.26\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.63 \\ 0.04 \\ 0.79\end{tabular} \\
 
%\midrule

% shifted pixel  (1) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.04 \\ -0.01 \\ -0.05\end{tabular} &  %1,2,3
% \begin{tabular}{@{}c@{}}0.36 \\ 1.0 \\ 0.26\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.16 \\ 0.14 \\ 0.11\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.67 \\ 0.04 \\ 0.7\end{tabular} \\
%\bottomrule
%\end{tabular}
%}
%\end{table}


%\begin{table}
%\centering
%\caption{Comparing data-based monitors for gtsrb dataset with different types of anomalies.}
%\resizebox{\columnwidth}{!}{%
%\label{table_anomaly_gtsrb}
%\begin{tabular}{llllllll}
%\toprule
%                Variation &                                             Method &                                                MCC &                                                FPR &                                                FNR &                                          Pr &                                             Re &                                           F1 \\
%\midrule
%    pixel trap  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%    \begin{tabular}{@{}c@{}}0.6 \\ -0.01 \\ -0.01\end{tabular} &  %1,2,2
%    \begin{tabular}{@{}c@{}}0.09 \\ 0.85 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.66 \\ 0.19 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.87 \\ 0.27 \\ 0.09\end{tabular} \\
    
%\midrule

% row add logic  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.02 \\ 0.03 \\ 0.02\end{tabular} &  %3,1,2
% \begin{tabular}{@{}c@{}}0.73 \\ 0.81 \\ 0.97\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.19 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.38 \\ 0.32 \\ 0.11\end{tabular} \\
 
% \midrule
 
% shifted pixel  (3) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.02 \\ 0.01 \\ 0.02\end{tabular} &  %1,2,1
% \begin{tabular}{@{}c@{}}0.69 \\ 0.83 \\ 0.97\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.2 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.42 \\ 0.29 \\ 0.11\end{tabular} \\
 
% \midrule
 
%    pixel trap  (1) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%    \begin{tabular}{@{}c@{}}0.19 \\ 0.01 \\ 0.01\end{tabular} &  %1,2,2
%    \begin{tabular}{@{}c@{}}0.47 \\ 0.83 \\ 0.97\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.27 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.61 \\ 0.28 \\ 0.1\end{tabular} \\
    
%\midrule

% row add logic  (1) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.0 \\ 0.0 \\ 0.11\end{tabular} &  %2,2,1
% \begin{tabular}{@{}c@{}}0.7 \\ 0.84 \\ 0.9\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.2 \\ 0.2 \\ 0.21\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 0.28 \\ 0.21\end{tabular} \\
 
% \midrule
 
% shifted pixel  (1) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.0 \\ 0.06 \\ 0.12\end{tabular} &  %3,2,1
% \begin{tabular}{@{}c@{}}0.7 \\ 0.77 \\ 0.89\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.2 \\ 0.21 \\ 0.21\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 0.35 \\ 0.23\end{tabular} \\
%\bottomrule
%\end{tabular}
%}
%\end{table}

==> sections/tables/noise_tables.tex <==
\begin{table}[htb!]
\centering
\caption{Comparing data-based monitors for CIFAR-10 and GTSRB datasets with \textbf{noise}.}
\resizebox{\columnwidth}{!}{%
\label{table_noise}
\begin{tabular}{llllllll}
\toprule
\multicolumn{8}{c} {CIFAR-10}\\
\toprule
Variation &                                             Method &                                                MCC &                                                FPR &                                                FNR &                                          Pr &                                             Re &                                           F1 \\
\midrule
     gaussian blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 \begin{tabular}{@{}c@{}}\textbf{0.29} \\ 0.0 \\ 0.13\end{tabular} &  %1,3,2
 \begin{tabular}{@{}c@{}}0.11 \\ 1.0 \\ \textbf{0.08}\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ \textbf{0.0} \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.39} \\ 0.14 \\ 0.28\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ \textbf{1.0} \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.82} \\ 0.04 \\ 0.8\end{tabular} \\
    
 \midrule
  
 zoom blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 \begin{tabular}{@{}c@{}}\textbf{0.47} \\ 0.0 \\ 0.1\end{tabular} &  %1,3,2
 \begin{tabular}{@{}c@{}}\textbf{0.03} \\ 1.0 \\ 0.1\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ \textbf{0.0} \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.69} \\ 0.14 \\ 0.24\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ \textbf{1.0} \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.88} \\ 0.04 \\ 0.79\end{tabular} \\
    
\midrule

 glass blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
  \begin{tabular}{@{}c@{}}\textbf{0.3} \\ 0.0 \\ 0.1\end{tabular} &  %1,3,2
  \begin{tabular}{@{}c@{}}\textbf{0.1} \\ 1.0 \\ 0.11\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ \textbf{0.0} \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.4} \\ 0.14 \\ 0.23\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ \textbf{1.0} \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.83} \\ 0.04 \\ 0.79\end{tabular} \\

\bottomrule
\bottomrule
\multicolumn{8}{c} {GTSRB}\\
\toprule
Variation &                                             Method &                                                MCC &                                                FPR &                                                FNR &                                          Pr &                                             Re &                                           F1 \\
\midrule
      gaussian blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 \begin{tabular}{@{}c@{}}-0.17 \\ 0.0 \\ \textbf{0.06}\end{tabular} &  %3,2,1
 \begin{tabular}{@{}c@{}}0.86 \\ \textbf{0.84} \\ 0.95\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.29} \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.17 \\ \textbf{0.2} \\ \textbf{0.2}\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ \textbf{0.98}\end{tabular} &  \begin{tabular}{@{}c@{}}0.24 \\ \textbf{0.27} \\ 0.14\end{tabular} \\
 
 \midrule
 
 zoom blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 \begin{tabular}{@{}c@{}}-0.11 \\ 0.0 \\ \textbf{0.02}\end{tabular} &  %3,2,1
 \begin{tabular}{@{}c@{}}\textbf{0.82} \\ 0.84 \\ 0.97\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ \textbf{0.02}\end{tabular} &  \begin{tabular}{@{}c@{}}0.17 \\ \textbf{0.2} \\ \textbf{0.2}\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ \textbf{0.98}\end{tabular} &  \begin{tabular}{@{}c@{}}\textbf{0.28} \\ \textbf{0.28} \\ 0.11\end{tabular} \\
 
 \midrule
 
 glass blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 \begin{tabular}{@{}c@{}}-0.11 \\ 0.01 \\ \textbf{0.06}\end{tabular} &  %3,2,1
 \begin{tabular}{@{}c@{}}\textbf{0.82} \\ 0.83 \\ 0.95\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ \textbf{0.02}\end{tabular} &  \begin{tabular}{@{}c@{}}0.17 \\ \textbf{0.2} \\ \textbf{0.2}\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ \textbf{0.98}\end{tabular} &  \begin{tabular}{@{}c@{}}0.28 \\ \textbf{0.29} \\ 0.14\end{tabular} \\
 
\bottomrule
\end{tabular}
}
\end{table}






%\begin{table}[htb!]
%\centering
%\caption{Comparing data-based monitors for cifar10 dataset with different types of noise.}
%\resizebox{\columnwidth}{!}{%
%\label{table_noise_cifar10}
%\begin{tabular}{llllllll}
%\toprule
%                    Variation &                                             Method &                                                MCC &                                                FPR &                                                FNR &                                          Pr &                                             Re &                                           F1 \\
%\midrule
%    gaussian noise  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%    \begin{tabular}{@{}c@{}}-0.03 \\ 0.0 \\ 0.0\end{tabular} &  %3,1,1
%    \begin{tabular}{@{}c@{}}0.45 \\ 1.0 \\ 1.0\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.0\end{tabular} &  \begin{tabular}{@{}c@{}}0.13 \\ 0.14 \\ 0.14\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 1.0\end{tabular} &  \begin{tabular}{@{}c@{}}0.6 \\ 0.04 \\ 0.04\end{tabular} \\
    
% \midrule
 
%    gaussian noise  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%    \begin{tabular}{@{}c@{}}-0.01 \\ 0.0 \\ 0.01\end{tabular} &  %3,2,1
%    \begin{tabular}{@{}c@{}}0.42 \\ 1.0 \\ 0.18\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.14 \\ 0.14 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.62 \\ 0.04 \\ 0.74\end{tabular} \\
    
% \midrule
 
%     impulse noise  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%     \begin{tabular}{@{}c@{}}-0.02 \\ 0.0 \\ 0.02\end{tabular} &  %3,2,1
%     \begin{tabular}{@{}c@{}}0.44 \\ 1.0 \\ 0.17\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.13 \\ 0.14 \\ 0.16\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.61 \\ 0.04 \\ 0.75\end{tabular} \\
    
%\midrule
     
%     impulse noise  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%     \begin{tabular}{@{}c@{}}-0.02 \\ 0.0 \\ 0.02\end{tabular} &  %3,2,1
%     \begin{tabular}{@{}c@{}}0.44 \\ 1.0 \\ 0.17\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.13 \\ 0.14 \\ 0.16\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.61 \\ 0.04 \\ 0.75\end{tabular} \\
     
% \midrule
 
%    shot noise  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%    \begin{tabular}{@{}c@{}}-0.02 \\ 0.0 \\ 0.03\end{tabular} &  %3,2,1
%    \begin{tabular}{@{}c@{}}0.44 \\ 1.0 \\ 0.16\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.13 \\ 0.14 \\ 0.17\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.61 \\ 0.04 \\ 0.76\end{tabular} \\
    
% \midrule
 
%shot noise  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}-0.04 \\ 0.0 \\ 0.0\end{tabular} &  %3,1,1
%\begin{tabular}{@{}c@{}}0.46 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.13 \\ 0.14 \\ 0.14\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.04 \\ 0.74\end{tabular} \\
    
%\midrule
 
%spatter  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}-0.02 \\ 0.01 \\ 0.01\end{tabular} &  %3,1,1
%\begin{tabular}{@{}c@{}}0.44 \\ 1.0 \\ 0.18\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.13 \\ 0.14 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.61 \\ 0.04 \\ 0.74\end{tabular} \\

%\midrule

%spatter  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}-0.01 \\ 0.01 \\ 0.01\end{tabular} &  %3,1,1
%\begin{tabular}{@{}c@{}}0.42 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.14 \\ 0.14 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.62 \\ 0.04 \\ 0.74\end{tabular} \\

% \midrule
 
% speckle noise  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.02 \\ 0.0 \\ 0.01\end{tabular} &  %3,2,1
% \begin{tabular}{@{}c@{}}0.44 \\ 0.84 \\ 0.18\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.16 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.13 \\ 0.2 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 0.84 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.61 \\ 0.28 \\ 0.74\end{tabular} \\
 
%  \midrule

% speckle noise  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.01 \\ 0.0 \\ 0.0\end{tabular} &  %1,2,2
% \begin{tabular}{@{}c@{}}0.4 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.15 \\ 0.14 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.64 \\ 0.04 \\ 0.74\end{tabular} \\
 
%  \midrule
  
% defocus blur  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.14 \\ 0.0 \\ 0.01\end{tabular} &  %1,3,2
% \begin{tabular}{@{}c@{}}0.23 \\ 1.0 \\ 0.18\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.23 \\ 0.14 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.75 \\ 0.04 \\ 0.74\end{tabular} \\
 
%  \midrule
  
% defocus blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.48 \\ 0.0 \\ 0.04\end{tabular} &  %1,3,2
% \begin{tabular}{@{}c@{}}0.03 \\ 1.0 \\ 0.16\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.7 \\ 0.14 \\ 0.17\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.88 \\ 0.04 \\ 0.76\end{tabular} \\
 
%  \midrule
  
% elastic transform  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.43 \\ 0.0 \\ 0.04\end{tabular} &  %1,3,2
% \begin{tabular}{@{}c@{}}0.04 \\ 1.0 \\ 0.15\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.6 \\ 0.14 \\ 0.18\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.87 \\ 0.04 \\ 0.76\end{tabular} \\
 
%  \midrule
  
% elastic transform  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.61 \\ 0.0 \\ 0.09\end{tabular} &  %1,3,2
% \begin{tabular}{@{}c@{}}0.0 \\ 1.0 \\ 0.11\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}1.0 \\ 0.14 \\ 0.23\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.9 \\ 0.04 \\ 0.78\end{tabular} \\
 
%  \midrule
  
% glass blur  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.06 \\ 0.0 \\ 0.05\end{tabular} &  %1,3,2
% \begin{tabular}{@{}c@{}}0.32 \\ 1.0 \\ 0.14\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.17 \\ 0.14 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.69 \\ 0.04 \\ 0.77\end{tabular} \\
 
%  \midrule
  
%  glass blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%  \begin{tabular}{@{}c@{}}0.3 \\ 0.0 \\ 0.1\end{tabular} &  %1,3,2
%  \begin{tabular}{@{}c@{}}0.1 \\ 1.0 \\ 0.11\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.4 \\ 0.14 \\ 0.23\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.83 \\ 0.04 \\ 0.79\end{tabular} \\
  
%  \midrule
  
%  zoom blur  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 % \begin{tabular}{@{}c@{}}0.49 \\ 0.0 \\ 0.07\end{tabular} &  %1,3,2
 % \begin{tabular}{@{}c@{}}0.03 \\ 1.0 \\ 0.13\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.72 \\ 0.14 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.88 \\ 0.04 \\ 0.77\end{tabular} \\
  
 % \midrule
  
 %zoom blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
 %\begin{tabular}{@{}c@{}}0.47 \\ 0.0 \\ 0.1\end{tabular} &  %1,3,2
 %\begin{tabular}{@{}c@{}}0.03 \\ 1.0 \\ 0.1\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.69 \\ 0.14 \\ 0.24\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.88 \\ 0.04 \\ 0.79\end{tabular} \\
 
 % \midrule
  
%gaussian blur  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}0.13 \\ 0.0 \\ 0.06\end{tabular} &  %1,3,2
%\begin{tabular}{@{}c@{}}0.24 \\ 1.0 \\ 0.13\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.22 \\ 0.14 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.74 \\ 0.04 \\ 0.77\end{tabular} \\

% \midrule
 
% gaussian blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.29 \\ 0.0 \\ 0.13\end{tabular} &  %1,3,2
% \begin{tabular}{@{}c@{}}0.11 \\ 1.0 \\ 0.08\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.0 \\ 0.81\end{tabular} &  \begin{tabular}{@{}c@{}}0.39 \\ 0.14 \\ 0.28\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 1.0 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.82 \\ 0.04 \\ 0.8\end{tabular} \\
%\bottomrule
%\end{tabular}
%}
%\end{table}





%\begin{table}
%\centering
%\caption{Comparing data-based monitors for gtsrb dataset with different types of noise.}
%\resizebox{\columnwidth}{!}{%
%\label{table_noise_gtsrb}
%\begin{tabular}{llllllll}
%\toprule
%                    Variation &                                             Method &                                                MCC &                                                FPR &                                                FNR &                                          Pr &                                             Re &                                           F1 \\
%\midrule
%gaussian noise  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}0.06 \\ 0.01 \\ 0.0\end{tabular} &  %1,2,3
%\begin{tabular}{@{}c@{}}0.63 \\ 0.83 \\ 0.84\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.16\end{tabular} &  \begin{tabular}{@{}c@{}}0.21 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.84\end{tabular} &  \begin{tabular}{@{}c@{}}0.47 \\ 0.28 \\ 0.28\end{tabular} \\
    
%\midrule

%gaussian noise  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}0.17 \\ 0.01 \\ 0.0\end{tabular} &  %1,2,3
%\begin{tabular}{@{}c@{}}0.5 \\ 0.83 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.26 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.59 \\ 0.29 \\ 0.1\end{tabular} \\

%\midrule

% impulse noise  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.09 \\ 0.01 \\ 0.0\end{tabular} &  %1,2,3
% \begin{tabular}{@{}c@{}}0.59 \\ 0.83 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.23 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.51 \\ 0.29 \\ 0.1\end{tabular} \\
 
% \midrule
 
% impulse noise  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.5 \\ 0.02 \\ -0.02\end{tabular} &  %1,2,3
% \begin{tabular}{@{}c@{}}0.15 \\ 0.82 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.53 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.83 \\ 0.3 \\ 0.09\end{tabular} \\
 
% \midrule
 
% shot noise  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}0.0 \\ 0.0 \\ -0.06\end{tabular} &  %1,1,3
% \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.99\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.2 \\ 0.2 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.41 \\ 0.28 \\ 0.07\end{tabular} \\
 
%\midrule

%shot noise  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}0.05 \\ 0.01 \\ -0.01\end{tabular} &  %1,1,3
%\begin{tabular}{@{}c@{}}0.64 \\ 0.83 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.21 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.47 \\ 0.28 \\ 0.09\end{tabular} \\

%\midrule

%spatter  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}0.65 \\ 0.05 \\ -0.01\end{tabular} &  %1,1,3
%\begin{tabular}{@{}c@{}}0.06 \\ 0.78 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.73 \\ 0.21 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.89 \\ 0.34 \\ 0.09\end{tabular} \\

%\midrule

%spatter  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}0.66 \\ 0.05 \\ -0.13\end{tabular} &  %1,1,3
%\begin{tabular}{@{}c@{}}0.06 \\ 0.79 \\ 1.0\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.74 \\ 0.21 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.89 \\ 0.34 \\ 0.06\end{tabular} \\

%\midrule

%speckle noise  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}0.01 \\ 0.0 \\ -0.12\end{tabular} &  %1,2,3
%\begin{tabular}{@{}c@{}}0.69 \\ 0.84 \\ 1.0\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.2 \\ 0.2 \\ 0.19\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.42 \\ 0.28 \\ 0.06\end{tabular} \\

%\midrule

%speckle noise  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}0.05 \\ 0.0 \\ -0.01\end{tabular} &  %1,2,3
%\begin{tabular}{@{}c@{}}0.65 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.21 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.46 \\ 0.28 \\ 0.09\end{tabular} \\

%\midrule

%defocus blur  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}-0.08 \\ 0.0 \\ -0.01\end{tabular} &  %3,1,2
%\begin{tabular}{@{}c@{}}0.79 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.18 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.31 \\ 0.28 \\ 0.09\end{tabular} \\

%\midrule

%defocus blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}-0.11 \\ 0.0 \\ 0.01\end{tabular} &  %3,2,1
%\begin{tabular}{@{}c@{}}0.81 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.17 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.28 \\ 0.1\end{tabular} \\

%\midrule

%elastic transform  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
%\begin{tabular}{@{}c@{}}-0.08 \\ 0.0 \\ 0.04\end{tabular} &  %3,2,1
%\begin{tabular}{@{}c@{}}0.79 \\ 0.84 \\ 0.96\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.18 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.32 \\ 0.28 \\ 0.13\end{tabular} \\

%\midrule

% elastic transform  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.09 \\ 0.01 \\ 0.04\end{tabular} &  %3,2,1
% \begin{tabular}{@{}c@{}}0.8 \\ 0.83 \\ 0.96\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.18 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.31 \\ 0.29 \\ 0.13\end{tabular} \\
 
% \midrule
 
% glass blur  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.07 \\ 0.01 \\ 0.02\end{tabular} &  %3,2,1
% \begin{tabular}{@{}c@{}}0.78 \\ 0.83 \\ 0.97\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.18 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.33 \\ 0.29 \\ 0.11\end{tabular} \\
 
% \midrule
 
% glass blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.11 \\ 0.01 \\ 0.06\end{tabular} &  %3,2,1
% \begin{tabular}{@{}c@{}}0.82 \\ 0.83 \\ 0.95\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.17 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.28 \\ 0.29 \\ 0.14\end{tabular} \\
 
% \midrule
 
% zoom blur  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.09 \\ 0.0 \\ 0.01\end{tabular} &  %3,2,1
% \begin{tabular}{@{}c@{}}0.8 \\ 0.84 \\ 0.97\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.18 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.31 \\ 0.28 \\ 0.1\end{tabular} \\
 
% \midrule
 
% zoom blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.11 \\ 0.0 \\ 0.02\end{tabular} &  %3,2,1
% \begin{tabular}{@{}c@{}}0.82 \\ 0.84 \\ 0.97\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.17 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.28 \\ 0.28 \\ 0.11\end{tabular} \\
 
% \midrule
 
% gaussian blur  (2) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.11 \\ 0.0 \\ 0.02\end{tabular} &  %3,2,1
% \begin{tabular}{@{}c@{}}0.82 \\ 0.84 \\ 0.97\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.17 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.28 \\ 0.28 \\ 0.11\end{tabular} \\
 
% \midrule
 
% gaussian blur  (5) &  \begin{tabular}{@{}c@{}}ALOOC \\ OOB \\ ODIN\end{tabular} &  
% \begin{tabular}{@{}c@{}}-0.17 \\ 0.0 \\ 0.06\end{tabular} &  %3,2,1
% \begin{tabular}{@{}c@{}}0.86 \\ 0.84 \\ 0.95\end{tabular} &  \begin{tabular}{@{}c@{}}0.29 \\ 0.16 \\ 0.02\end{tabular} &  \begin{tabular}{@{}c@{}}0.17 \\ 0.2 \\ 0.2\end{tabular} &  \begin{tabular}{@{}c@{}}0.71 \\ 0.84 \\ 0.98\end{tabular} &  \begin{tabular}{@{}c@{}}0.24 \\ 0.27 \\ 0.14\end{tabular} \\
%\bottomrule
%\end{tabular}
%}
%\end{table}

==> sections/tables/processing_time_tables.tex <==
\begin{table}[htb!]
\centering
\caption{Time impact of ALOOC-based monitors per instance in seconds.}
\label{table_alooc_time_1}
\begin{tabular}{llll}
\toprule

Dataset & Prediction &           Monitoring &              SUT \\

\midrule
        GTSRB-BTSC &  0.04275 (38.26\%) &  0.06876 (61.53\%) &  0.11174 \\
      %& rmsprop &  0.04318 (38.38\%) &  0.06911 (61.42\%) &  0.11253 \\
%\midrule

%\midrule
	GTSRB-CIFAR &  0.00194 (5.95\%) &  0.03063 (93.72\%) &  0.03268 \\
    %& rmsprop &  0.00187 (5.99\%) &  0.02924 (93.69\%) &  0.03121 \\
%\midrule

%\midrule
	CIFAR-GTSRB &  0.0006 (6.13\%) &  0.0092 (93.55\%) &  0.00984 \\
    %& rmsprop &  0.00061 (6.16\%) &  0.0092 (93.53\%) &  0.00984 \\

\bottomrule
\end{tabular}
\end{table}

\begin{table}[htb!]
\centering
\caption{Time impact of OOB-based monitors per instance in seconds.}
\label{table_oob_time_1}
\begin{tabular}{llll}
\toprule

Dataset & Prediction &           Monitoring &              SUT \\
\midrule
       GTSRB-BTSC & 0.00702 (3.07\%) &  0.22173 (96.89\%) &  0.22884 \\
	GTSRB-CIFAR & 0.00218 (3.96\%) &  0.05291 (96.0\%) &  0.05511 \\
	CIFAR-GTSRB & 0.00077 (3.03\%) &  0.02469 (96.93\%) &  0.02547 \\

\bottomrule
\end{tabular}
\end{table}


\begin{table}[htb!]
\centering
\caption{Time impact of ODIN-based monitors per instance in seconds.}
\label{table_odin_time_1}
\begin{tabular}{llll}
\toprule

Dataset & Prediction &           Monitoring &              SUT \\
\midrule
       GTSRB-BTSC & 0.00139 (15.17\%) &  0.00727 (79.36\%) &  0.00916 \\
	GTSRB-CIFAR & 0.00015 (15.95\%) &  0.00074 (78.72\%) &  0.00094 \\
	CIFAR-GTSRB & 0.00051 (15.31\%) &  0.00265 (79.57\%) &  0.00333 \\

\bottomrule
\end{tabular}
\end{table}
